SimPB: A Single Model for 2D and 3D Object Detection from Multiple Cameras

The field of autonomous driving has attracted considerable interest in approaches that directly infer 3D objects in the Bird's Eye View (BEV) from multiple cameras. Some attempts have also explored utilizing 2D detectors from single images to enhance the performance of 3D detection. However, these approaches rely on a two-stage process with separate detectors, where the 2D detection results are utilized only once for token selection or query initialization. In this paper, we present a single model termed SimPB, which simultaneously detects 2D objects in the perspective view and 3D objects in the BEV space from multiple cameras. To achieve this, we introduce a hybrid decoder consisting of several multi-view 2D decoder layers and several 3D decoder layers, specifically designed for their respective detection tasks. A Dynamic Query Allocation module and an Adaptive Query Aggregation module are proposed to continuously update and refine the interaction between 2D and 3D results, in a cyclic 3D-2D-3D manner. Additionally, Query-group Attention is utilized to strengthen the interaction among 2D queries within each camera group. In the experiments, we evaluate our method on the nuScenes dataset and demonstrate promising results for both 2D and 3D detection tasks. Our code is available at: https://github.com/nullmax-vision/SimPB.

==> table/5_ablation_allocation.tex <==
\begin{table}
\centering
\caption{Ablation studies on query allocation mechanism.}
\begin{tabular}{l|cc}
    \toprule
    Allocation Strategy & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\  \\
    \midrule
    Uniform                               & 0.365    & 0.474        \\
    Object Center                         & 0.410    & 0.515        \\
    Object Center + Front-Rear Point      & 0.414    & 0.520        \\
    \rowcolor{gray!15}
    Object Center + Anchor Corner \qquad  & \textbf{0.421}    & \textbf{0.527}        \\
    \bottomrule
\end{tabular}
\label{tab:ablation_allocation}
\end{table}

==> table/6_ablation_aggregation.tex <==
\begin{table}
    \centering
    \caption{Ablation studies on query aggregation mechanism.}
    \begin{tabular}{l|cc}
    \toprule
    Aggregation Strategy \ & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\  \\
    \midrule
    Cross-Attention                \  & 0.365     & 0.474    \\
    Cross-Attention + Supervision  \  & 0.399     & 0.495    \\
    Query Fusion                   \  & 0.389     & 0.489    \\
    \rowcolor{gray!15}
    Query Fusion + Supervision     \  & \textbf{0.421}     & \textbf{0.527}    \\
    % Self-Attn + Reweight     \  & -     & -    \\
    % \rowcolor{gray!15}
    % Self-Attn + Reweight + Supervision  \  & \textbf{0.421}     & \textbf{0.514}    \\
    \bottomrule
\end{tabular}
\label{tab:ablation_aggregation}
\end{table}





==> table/7_ablation_loss.tex <==
\begin{table}
\centering
\caption{The ablation studies of camera observation loss.}
\begin{tabular}{@{}l|ccc@{}}
    \toprule
    \ \ $\lambda_{alpha}$   & \ mAP$\uparrow$\,  & \,NDS$\uparrow$ \, & \ mAOE$\downarrow$ \\
    \midrule
    \ \ -            & 0.421          & 0.514 & 0.611  \\
    \ \ 0.25         & \textbf{0.425} & 0.519 & 0.582  \\
    \rowcolor{gray!15}
    \ \ 0.50         & 0.421 & \textbf{0.527} & 0.492  \\
    \ \ 1.00         & 0.418 & 0.523 & \textbf{0.465}  \\
    
    \bottomrule
\end{tabular}
\label{tab:ablation_loss}
\end{table}

==> table/8_ablation_integration.tex <==
\begin{table}
\centering
\caption{Integrate our SimPB to other methods.}
\begin{tabular}{l|llc}
    \toprule
    Method \qquad \qquad \qquad  & \ mAP$\uparrow$\,  & \,NDS$\uparrow$\ \\
    \midrule
    DETR3D~\cite{DETR3D}         & \ 0.258   & 0.306   \\
    \rowcolor{gray!15}
    DETR3D-SimPB                 & \ 0.282 (+\hlr{0.024})  & 0.358 (+\hlr{0.052}) \\
    \midrule
    Sparse4Dv2~\cite{Sparse4Dv2} & \ 0.367  & 0.450  \\
    \rowcolor{gray!15}
    Sparse4Dv2-SimPB \           & \ 0.398 (+\hlr{0.031})  & 0.480 (+\hlr{0.030}) \\
    \bottomrule
\end{tabular}
\label{tab:ablation_integrate}
\end{table}

